Lightweight Modality Adaptation to Sequential Recommendation via Correlation Supervision

In Sequential Recommenders (SR), encoding and utilizing modalities in an end-to-end manner is costly in terms of modality encoder sizes. Two-stage approaches can mitigate such concerns, but they suffer from poor performance due to modality forgetting, where the sequential objective overshadows modality representation. We propose a lightweight knowledge distillation solution that preserves both merits: retaining modality information and maintaining high efficiency. Specifically, we introduce a novel method that enhances the learning of embeddings in SR through the supervision of modality correlations. The supervision signals are distilled from the original modality representations, including both (1) holistic correlations, which quantify their overall associations, and (2) dissected correlation types, which refine their relationship facets (honing in on specific aspects like color or shape consistency). To further address the issue of modality forgetting, we propose an asynchronous learning step, allowing the original information to be retained longer for training the representation learning module. Our approach is compatible with various backbone architectures and outperforms the top baselines by 6.8% on average. We empirically demonstrate that preserving original feature associations from modality encoders significantly boosts task-specific recommendation adaptation. Additionally, we find that larger modality encoders (e.g., Large Language Models) contain richer feature sets which necessitate more fine-grained modeling to reach their full performance potential.

==> review/comments.ecir.tex <==
# Reviewer1:

1. The authors should consider sharing more relevant background on other works that study the problem of modality forgetting. If there are no other works, the authors should clearly themselves as the first researchers to study this direction.

> Accept. We will state we are the first propose this problem.
> 

2. The authors can consider sharing more intuition behind fine-grained correlations in CDL. Even thought the experimental results show their effectiveness, the authors should consider showing some qualitative examples where presence of both correlations improves ranking performance.

> Pending
> 

3. The authors conduct no ablations on the need of the linear Autoencoder for dimensionality reduction. This seems kind of counter-intuitive because latest pretrained modality encoders are usually as it is and have demonstrated strong performance on their high dimension representations.

> The comments make sense. But we use AE because it can convert original representations into the ones with more distinctive features. I will highlight it in Modality Correlation Distillation part.
> 

# Reviewer2:

1. Would have preferred to have seen some of the more recent vision + language models.

> Ignore
> 

2. For the vector quantization, how was x chosen and why?

> Accept. Mentioned it in page 6, Modality Correlation Distillation
> 

3. A few examples on where the recommendations work due to the proposed method, and where it fails would have been helpful.

> Pending
> 

# Reviewer3:

- The main contribution is the development of the KDSR model. While innovative, the paper does not explore a broader range of methodologies or theoretical advancements in the field of Sequential Recommenders.
    
    > Ignore
    > 
- The paper proposes a method to avoid modality forgetting, but there could be a stronger theoretical or empirical justification for why this method is effective in addressing this specific issue.
    
    > Ignore
    > 
- The research relies on just two datasets (Amazon review and MovieLens). The limited variety might not adequately represent the diverse real-world scenarios, affecting the generalizability of the findings.
    
    > Reject. Many previous work did the modality-enriched experiments on just these two datasets as well.
    >

==> review/comments.original.ecir.tex <==
-------------------------  METAREVIEW  ------------------------
The paper generally received positive reviews and the recommendation is to accept. There are, however, issues mentioned in the reviews that should be addressed in the final version.



----------------------- REVIEW 1 ---------------------
SUBMISSION: 50
TITLE: Lightweight Modality Adaptation to Sequential Recommendation via Correlation Supervision
AUTHORS: Hengchang Hu, Qijiong Liu, Chuang Li and Min-Yen Kan

----------- Relevance to ECIR -----------
SCORE: 2 (an IR conference is the natural place for this paper)
----------- Main contribution -----------
The paper has following primary contributions:
1. They demonstrate the problem of modality forgetting in typical two stage sequential recommendation models.
2. They propose a novel knowledge distillation framework, combining coarse and fine-grained correlation supervision in embedding learning, that improves the retainability of modality information.
3. Conduct thorough experiments to show the improvement contributed by their approach. They also conduct several ablations to demonstrate that their solution can keep adapting to evolving state of the art modality encoders.
----------- Strengths -----------
Strengths:
1. The paper is very well written. The authors are able to share the relevant context, problem statement, their proposed framework, experimental results and ablations fluently and lucidly.
2. The authors demonstrate that their proposed framework consistently improves performance over the baseline for all the 5 datasets, thereby validating their hypothesis and the soundness of their approach.
3. The authors perform detailed ablation experiments across all the components in their proposed correlation distillation learning setup. Particularly, they demonstrate the effectiveness of using both coarse-grained and the fine-grained features, which is quite pivotal to this paper.
4. The authors also demonstrate how their results are impacted by increasing modality encoder sophistication. Their results show that performance does improve with better encoders. This result is extremely useful in modern times where modality encoders are getting much larger and sophisticated.
----------- Limitations -----------
Limitations:
1. The authors should consider sharing more relevant background on other works that study the problem of modality forgetting. If there are no other works, the authors should clearly themselves as the first researchers to study this direction.
2. The authors can consider sharing more intuition behind fine-grained correlations in CDL. Even thought the experimental results show their effectiveness, the authors should consider showing some qualitative examples where presence of both correlations improves ranking performance.
3. The authors conduct no ablations on the need of the linear Autoencoder for dimensionality reduction. This seems kind of counter-intuitive because latest pretrained modality encoders are usually as it is and have demonstrated strong performance on their high dimension representations.
----------- Detailed comments -----------
In this paper, the authors study the problem of modality forgetting in two stage sequential recommendation systems. They demonstrate how modality-specific embeddings are diluted in such systems and the models eventually end up learning purely sequential representations. In order to address this issue, the authors propose a knowledge distillation solution that makes use of both coarse and fine-grained correlation supervision for representation learning. To demonstrate the effectiveness of their approach, the authors experiment on 5 datasets and show that their proposed approach consistently improves over the baseline models for all of them. The authors also conduct comprehensive ablations to demonstrate the importance of each of their proposed component in the KD framework and the overall generality of their approach when used with different representation learning backbones and sophisticated modality encoders.
 
Overall, the paper is very well written and clearly describes the authors' ideas and approaches. The contributions made by the paper are very relevant in current times where researchers are increasingly leveraging representations from large pretrained modality encoders. The authors' approach enables sequential recommendation practitioners and researchers to effectively use these large pretrained models with two stage methods. I believe the paper will make a good addition to the conference.


Strengths:
1. The paper is very well written. The authors are able to share the relevant context, problem statement, their proposed framework, experimental results and ablations fluently and lucidly.
2. The authors demonstrate that their proposed framework consistently improves performance over the baseline for all the 5 datasets, thereby validating their hypothesis and the soundness of their approach.
3. The authors perform detailed ablation experiments across all the components in their proposed correlation distillation learning setup. Particularly                                             
   , they demonstrate the effectiveness of using both coarse-grained and the fine-grained features, which is quite pivotal to this paper.
4. The authors also demonstrate how their results are impacted by increasing modality encoder sophistication. Their results show that performance does improve with better encoders. This result is extremely useful in modern times where modality encoders are getting much larger and sophisticated.

Limitations:
1. The authors should consider sharing more relevant background on other works that study the problem of modality forgetting. If there are no other works, the authors should clearly themselves as the first researchers to study this direction.
2. The authors can consider sharing more intuition behind fine-grained correlations in CDL. Even thought the experimental results show their effectiveness, the authors should consider showing some qualitative examples where presence of both correlations improves ranking performance.
3. The authors conduct no ablations on the need of the linear Autoencoder for dimensionality reduction. This seems kind of counter-intuitive because latest pretrained modality encoders are usually as it is and have demonstrated strong performance on their high dimension representations.

Typos
1. Typo on page 2 in 1st paragraph of Related Works. "effectiveness of the apply" -> "effectiveness of the application".
----------- Impact of Contributions -----------
SCORE: 4 (Some of the ideas, results, or resources will substantially help other people's ongoing research)
----------- Originality of the work -----------
SCORE: 4 (Incremental but important: Although it is an incremental improvement, its impact is significant.)
----------- Technical Soundness -----------
SCORE: 4 (The technical facts are appropriately described but there are some minor errors or omissions)
----------- Quality of Presentation -----------
SCORE: 4 (The essential content is complete and the paper is understandable to most readers)
----------- Adequacy of Citations -----------
SCORE: 4 (The relevant publications are cited appropriately but the discussion could be more comprehensive or insightful)
----------- Reproducibility -----------
SCORE: 5 (Fully replicable: the experimental setup is fully transparent, described in detail, and the data is publicly available)
----------- Expertise -----------
SCORE: 3 (I have worked on related topics and have a good general understanding of the area)
----------- Recommendation -----------
SCORE: 2 (accept)



----------------------- REVIEW 2 ---------------------
SUBMISSION: 50
TITLE: Lightweight Modality Adaptation to Sequential Recommendation via Correlation Supervision
AUTHORS: Hengchang Hu, Qijiong Liu, Chuang Li and Min-Yen Kan

----------- Relevance to ECIR -----------
SCORE: 1 (not core-IR but still a good fit)
----------- Main contribution -----------
Suggesting an approach to preserve modality information for downstream sequential recommendation tasks.
----------- Strengths -----------
1. Nice problem motivation and description.
2. The correlation approaches for preserving coarse and fine-grained relationships.
3. The asynchronous training strategy for this problem.
----------- Limitations -----------
1. Would have preferred to have seen some of the more recent vision + language models.
2. For the vector quantization, how was x chosen and why?
3. A few examples on where the recommendations work due to the proposed method, and where it fails would have been helpful.
----------- Detailed comments -----------
The core idea of the paper is that in SR tasks, modality information that is generally retrieved from some encoder is diluted to a point, where they over-adapt to sequential correlations. So they authors suggest an idea, where-in they preserve information about the original modality, but focussing on preserving the correlations between items (using their modality embeddings.) This is a very nice approach, and intuitively makes a lot of sense, though the implementation seems a little more complicated. I am happy to accept this work, as the approaches, experiments and the metrics they report all make sense to me. A few minor thoughts as I was reading the paper:

1. A graph with increasing sequence length could show where the performance starts to taper off. It's pretty obv, at this point, for almost any sequence oriented  tasks, performance degrades over large sequences. So would have been nice to see a graph to understand at what point performance starts to drop.
2. For the vector quantization, how was x chosen? Were different values considered, and how did the performance change based on this value?
3. You could have used some of the more recent vision + language transformers. Most approaches are becoming nullified as soon as we get embeddings from these very large models, so since you didn’t use any of them, the question remains if your current approaches would help or just go away with these much larger models. You do refer to [52], but seem to be using [9,37] (referring to these from section 3.1)
----------- Impact of Contributions -----------
SCORE: 4 (Some of the ideas, results, or resources will substantially help other people's ongoing research)
----------- Originality of the work -----------
SCORE: 4 (Incremental but important: Although it is an incremental improvement, its impact is significant.)
----------- Technical Soundness -----------
SCORE: 4 (The technical facts are appropriately described but there are some minor errors or omissions)
----------- Quality of Presentation -----------
SCORE: 4 (The essential content is complete and the paper is understandable to most readers)
----------- Adequacy of Citations -----------
SCORE: 4 (The relevant publications are cited appropriately but the discussion could be more comprehensive or insightful)
----------- Reproducibility -----------
SCORE: 4 (The experiments could be reproduced: the experimental setup is clear, the data is described in detail, but is not available outside of the authors' organization)
----------- Expertise -----------
SCORE: 3 (I have worked on related topics and have a good general understanding of the area)
----------- Recommendation -----------
SCORE: 2 (accept)



----------------------- REVIEW 3 ---------------------
SUBMISSION: 50
TITLE: Lightweight Modality Adaptation to Sequential Recommendation via Correlation Supervision
AUTHORS: Hengchang Hu, Qijiong Liu, Chuang Li and Min-Yen Kan

----------- Relevance to ECIR -----------
SCORE: 2 (an IR conference is the natural place for this paper)
----------- Main contribution -----------
The authors introduce a lightweight knowledge distillation framework for SR, namely Knowledge Distillation for Modality-enriched Sequential Recommendation (KDSR). This method effectively balances the retention of original modality information into the model's representation while optimizing for sequential recommendation with high efficiency, in a two-stage training of SRs. It demonstrates compatibility with various SR architectures and larger modality encoders and outperforms previous methods.
----------- Strengths -----------
- The proposed KDSR framework is a novel approach, particularly in using knowledge distillation to retain modality correlations.
- The authors carry out comprehensive experiments across various scenarios, providing evidence of the method's effectiveness.
- The framework’s compatibility with multiple encoder architectures and various SR backbones is a significant advantage, especially given the rapid evolution in the size and complexity of these encoders.
----------- Limitations -----------
- The main contribution is the development of the KDSR model. While innovative, the paper does not explore a broader range of methodologies or theoretical advancements in the field of Sequential Recommenders.
- The paper proposes a method to avoid modality forgetting, but there could be a stronger theoretical or empirical justification for why this method is effective in addressing this specific issue.
- The research relies on just two datasets (Amazon review and MovieLens). The limited variety might not adequately represent the diverse real-world scenarios, affecting the generalizability of the findings.
----------- Detailed comments -----------
The paper is well-written and follows a clear flow.

The methodology section is well-structured and detailed, providing a clear explanation of the approach. However, it might benefit from a more explicit discussion on how the proposed method improves upon existing knowledge distillation techniques in SR.

The authors carry out an extensive experimental setup and a notable comparison with existing baselines. However, the paper could provide more insights into the scalability of the proposed method, especially in real-world scenarios with large datasets and user bases.

In summary, the proposed method shows promise, and with further exploration, especially in the areas mentioned, it could lead to significant advancements in the field, especially overlooking the benefits of future research in integrating deeper layers.
----------- Impact of Contributions -----------
SCORE: 4 (Some of the ideas, results, or resources will substantially help other people's ongoing research)
----------- Originality of the work -----------
SCORE: 5 (Truly novel and impactful: New ideas and validation of those which will most likely be impactful.)
----------- Technical Soundness -----------
SCORE: 5 (There are no technical shortcomings or omissions)
----------- Quality of Presentation -----------
SCORE: 5 (Well-written in every aspect)
----------- Adequacy of Citations -----------
SCORE: 4 (The relevant publications are cited appropriately but the discussion could be more comprehensive or insightful)
----------- Reproducibility -----------
SCORE: 4 (The experiments could be reproduced: the experimental setup is clear, the data is described in detail, but is not available outside of the authors' organization)
----------- Expertise -----------
SCORE: 2 (I have a good general understanding of the area)
----------- Recommendation -----------
SCORE: 2 (accept)

==> sec/approach_version1.tex <==
\section{Methodology}

\textbf{Problem Formulation.}
The conventional sequential recommendation aims to predict the next item $v$ a user $u$ is likely to consume, based on their historical interactions $\{v_1, \dots, v_m\}$.
Extending this, Modality-enhanced Sequential Recommendation (MSR) considers item modalities within the sequence to refine this predictive function. Specifically, the objective is to acquire a function $f: \{(v_1,a_1,b_1), \dots, (v_m, a_m, b_m) \} \rightarrow v$,
where $a$/$b$ denotes the modality features (image or text) and $a_i$/$b_i$ indicates the modality of item $v_i$ respectively.

% The goal of conventional \textit{sequential recommendation} can be stated as follows: Given the historical interaction data $\mathbf{H}_u: \{v_1, v_2, \dots, v_m\}$ of user $u$, the objective is to acquire a function $f: \{v_1, v_2, \dots, v_m\} \rightarrow v$ that can predict the next item $v$ that the user is highly likely to consume. 
% Building upon that, modality-enhanced sequential recommendation (MSR) takes into account the modality of items within the sequence, and target to a function that,
% \begin{equation}
%     g: \left\{
%     \begin{aligned}
%     & \mathbf{v}:\{v_1, v_2, \dots, v_m\}, \\
%     & \mathbf{a}:\{a_1, a_2, \dots, a_m\}. 
%     \end{aligned}
%     \right\}
%     \rightarrow
%     \left\{
%     \begin{aligned}
%     & v \\
%     & a 
%     \end{aligned}
%     \right\}
% \end{equation}
% where $a$ denotes the modality features (image or text) we took into consideration.
% Correspondingly, $a_i$ indicates the modality of item $v_i$ respectively.


% \subsection{Base Model of MSR}
\vspace{0.4em}
\noindent \textbf{Base Model of MSR.}
Most existing MSR methods adhere to an Embedding, Representation learning, and Prediction paradigm, which we term as the base model in this section.

\vspace{0.5em}
% \noindent \textit{Initial Embedding.}
\noindent \textit{Encoding.}


Item ID features $v$ are initially represented as integer index values and can be converted into low-dimensional, dense real-value vectors $\mathbf{e}_v$ using a randomly initialized embedding table. Modality $a$'s embeddings often involve directly using extracted features $\mathbf{m}_a$ and representing them as feature vectors $\mathbf{e}_a=\mathbf{m}_a$, through modality encoders \cite{he2016deep,raffel2020exploring}.

\vspace{0.5em}
\noindent 
\textit{Representation Learning.}
Several prior studies have focused on designing network architectures to model feature interactions and generate the overall sequence representation $\mathbf{P}$. Using the representation learning function $g$, this is given by:
\begin{equation}
    \mathbf{P} = g(\mathbf{(e_{v_1},e_{a_1}, e_{b_1}), (e_{v_2},e_{a_2}, e_{b_2}),...,(e_{v_m},e_{a_m}, e_{b_m})})
\end{equation}

\vspace{0.5em}
\noindent 
\textit{Prediction.}
The widely-used scoring method involves matching the learned user representation $\mathbf{P}$ with candidate items $\mathbf{e}_{v}$ using the dot product $\hat{y} = \mathbf{P} \cdot \mathbf{e}_{v}^\top$.
% \begin{equation}
% \hat{y} = \mathbf{P} \cdot \mathbf{e}_{v}^\top
% \end{equation}
During training, the model measures the differences between the ground-truth $y$ and the predicted score $\hat{y}$ using the cross-entropy loss \cite{kang2018self}, denoted as $\mathcal{L}^{RS}(y,\hat{y})$.


\subsection{Overall Framework of Knowledge Distillation for MSR}
\label{sec:pf_basemodel}

\holden{Shrink}

% 本文主要关注于MSR的encoding部分，如上所示，它主要包括两个步骤:

MSR consists of two core modules: the modality encoding module $a \rightarrow \mathbf{m}_a$, which represents modalities with training on large pertaining datasets; and the modality utilization module $\mathbf{m}_a \rightarrow \mathbf{e}_a$, which applies these pretrained representations to recommendation tasks.
However, as the training progresses, $e_a$ will gradually deviate from $m_a$, leading to the loss of modality-specific knowledge of the original feature $a$.


To fill the gap, we use a common teacher-student paradigm.
As shown in Figure~\ref{fig:framework} (left),
the teacher model distills correlations knowledge among modalities from the encoding module and then uses it to supervise the student model in the utilization module. 
In the training phase, the teacher model utilizes its capabilities to guide the student model, providing valuable feedback and helping it to learn from its errors. In the inference phase, the teacher model is no longer necessary, and the improved student model is employed to make predictions.

% \subsubsection{Teacher Model -- Modality Correlation Extraction} 
\textit{Teacher Model -- Modality Correlation Distillation.} 
Formally, let ${(m_i, m_j, r_{ij})}_{i=1}^N$ be the set of data pairs and corresponding relationships. In this context, the teacher model aims to predict the relationship $r{ij}$ based on the input pairs $(m_i, m_j)$ through the function $f^T(m_i, m_j) = r_{ij}$. In this notation, $m$ represents individual modality features, and $r$ captures their intrinsic correlations.


\textit{Student Model -- Modality Correlation Learning.} 
Similarly, the student model aims to predict the distilled correlations based on the updated modality embeddings. Specifically, the function $f^S(e_i, e_j)$ is designed to estimate $r_{ij}$, where $e_i$ and $e_j$ are the updated embeddings for the modalities in question.
During the training phase, the objective of the student model is to assist in recommendation tasks. This is achieved by minimizing the discrepancy between the outputs generated by the teacher model and those produced by the student model. Formally, the model seeks to minimize the difference between $f^T(m_i, m_j)$ and $f^S(e_i, e_j)$.


\begin{figure}[t]
    \setlength{\abovecaptionskip}{-0cm}
    \setlength{\belowcaptionskip}{-0.5cm}
    \centering
    \includegraphics[width=0.97\textwidth]{fig/framework.png}
    \caption{(left) Framework of modality-enrich recommendation. (right) Correlation distillation learning module \holden{Add an autoencoder as distillation layer in righthand side; illustrate the color meanings}.}
    \label{fig:framework}
\end{figure}

% Our paper presents a novel plug-in -- Correlation Distillation (CD) for use with the Base Model, which additionally constrains the correlation among modalities in the base model embedding. As depicted in Figure~\ref{fig:framework}, the Teacher model harnesses abstract knowledge to link modality correlations. Meanwhile, the Student model focuses on learning these distilled correlations for the recommendation system.
% In this section, we first outline the implementation of the unsupervised correlation extraction, i.e., the teacher model. Following that, we explain how these correlations guide the representation of modalities within the embedding space.

\subsection{Modality Correlation Learning}
\holden{Shrink}

\subsubsection{Modality Correlation Distillation.}
As depicted on the right side of Figure~\ref{fig:framework}, the first step is to distill coarse-grained and fine-grained supervision signals to flexibly control the correlation learning for modality embedding. Specifically, for each paired modal vectors $(m_i,m_j)$, the teacher model predicts:

\textit{Holistic modality correlation scores $f^T_{s}: \xi(m_i,m_j) \rightarrow r_{ij}$.}
An intuitive unsupervised method is to use a correlation scoring function $\xi$ to measure the overall difference (i.e., the continuous value $r$) between paired modal representations.
For instance, when using cosine similarity as the scoring function, it's calculated as the cosine of the angle between vectors $m_i$ and $m_j$, denoted as $\xi(m_i,m_j)=\text{cos}(\theta_{m_i, m_j})$, focusing on vector direction while ignoring magnitude. We provide both distance-based and similarity-based methods for correlation assessment $\xi$. Given the pivotal role of scoring functions in our study, they will be evaluated in our experiment part.


\vspace{0.5em}
% \noindent 
\textit{Dissected modality correlation codes $f^T_c: \pi(m_i,m_j) \rightarrow c_{ij}$.}
Considering direct vector-wise operations $\xi$ on their vectors are overly simplistic, we provide more fine-grained discrete correlation signals $c$ distillation through process $\pi$.
Modality vectors often encode diverse features like color and shape, necessitating a nuanced approach to fully capture their intrinsic relationships. For example, both (\textit{black-suit}, \textit{black-tie}) and (\textit{black-suit}, \textit{yellow-suit}) pairs may yield high holistic correlation scores, yet the specific attributes contributing to these scores vary. Hence, it's vital to encapsulate these unique correlation patterns into discrete \textit{correlation codes} for more targeted learning.

\begin{enumerate}[label=\roman*.]
    \item Correlation vectorization: 
            Instead of using a single scalar value $r_{i,j}$  to encapsulate the correlation between item modalities  $m_{a_i}$ and $m_{a_j}$, we propose employing a vector $\mathbb{r}_{i,j}$ to capture these relationships in a more fine-grained manner.
            Inspired by the concept of Product Quantization (PQ) \cite{jegou2010product}, we regard each sub-vector as a distinct yet meaningful segment. In this framework, we assume that different positions in the element correspond to unique, meaningful features.
            To begin, we decompose the modality representation vector $m_a$ into $D$ sub-vectors, denoted as $[m_{a,1}, ..., m_{a,D}]$. Following this, we compute the correlation scores (similarity or distance-based) between each sub-vector in $m_{a_i}$ and its counterpart in  $m_{a_j}$. Next, we concatenate these computed metrics to derive correlation vectors. Mathematically, this is expressed as $\mathbb{r}_{i,j} = [\mathbb{r}_{ij,1},...,\mathbb{r}_{ij,D}] = [\xi(m_{a_i,1},m_{a_j,1}), ..., \xi(m_{a_i,D},m_{a_j,D})]$. This methodology enables us to more accurately capture the nuanced relationships between the meaningful segments of the vectors. 
            % As a result, we obtain a comprehensive set of correlation vectors for each pair of items, organized in a tensor of shape $\mathbb{R}^{N \times N \times D}$.
    \item  Vector quantization: 
            The modality spaces produced by the modality encoder and those in the embedding space for SR are not strictly one-to-one aligned. To address this, we propose quantifying the $N \times N$ correlation vectors, $\{\mathbb{r}\}$, into correlation codes using Vector Quantization (VQ) \cite{hou2023learning}, a classic technique from signal processing.
            Initially, we create a codebook, an array of $K$ vectors, where $K$ is a predefined cluster count. Each \textit{codeword} in the codebook represents a potential state for a correlation. The codebook, typically initialized randomly, is refined using training data to better fit the input vector distribution.
            Next, we map each vector in our correlation distribution $C$ to its closest codeword, commonly using Euclidean distance as the metric.
            This converts $C$ from $\mathbb{R}^{N \times N \times D}$ to $\mathbb{R}^{N \times N \times 1}$, where each entry now holds an index value between $1$ and $K$, corresponding to the closest codeword.
\end{enumerate}

By the steps above, closely related correlation patterns in the original space are likely to be mapped to the same codeword, thereby clustering similar correlations. Meanwhile, this enables nuanced distinctions between varied patterns, such as "similar color, different shape" and "similar shape, different color," through unique codewords, offering more refined relationships.

% \subsection{Representation Learning}
% Building upon the base model mentioned in Section~\ref{sec:pf_basemodel}, we adopt a decomposed representation approach. This means the ID representing the collaborative information of the item and the modality information representing the features of the item itself are depicted by different vectors.

% Here, it's worth mentioning that in sequence modeling, these decomposed representations intertwine through various fusion methods -- including early fusion, late fusion, and overall fusion. These terms denote whether the fusion of modality features and ID features occurs before or after sequence modeling.

% Let's consider early fusion as an example. For each item, we merge its representations first, denoted as $e_i=merge(e_{v_i},e_{a_i})$, where we use a simple concatenation function for the merge.
% Given the historical interacted item sequence $H_u$ for each user, the representation learning module is responsible for modeling their relationship and producing the updated representation for each item, i.e., $X([e_1,e_2,...,e_n])=[h_1,h_2,...,h_n]$.
% The sequential modeling function $X$ can be any of the following: \textit{Transformer} (SASRec \cite{}), \textit{GRU} (GRU4Rec \cite{}), or a more \textit{intricate graph approach} (RGAT \cite{}).


\subsubsection{Distilled Correlation Learning}
To enforce the consistency of correlations within embeddings $E$ and modality representation $M$, we use a teacher-student framework. This aims to optimize a lighter student network to approximate the results from a heavier teacher model, aiding in tasks like neural network compression.
In the student model, we evaluate the correlation between two items based on their proximity, represented by holistic correlation, and their directional attributes, refined by dissected correlation codes. The details are shown as follows.

% \vspace{0.5em}
\noindent \textit{Holistic correlation learning.}
In the student model, the correlation between two items $v_i$ and $v_j$ is transformed through their original embeddings, as shown in:
\begin{equation}
    r^{'}_{ij} = \xi \left(g_\phi (a_{i}), g_\phi (a_{j}) \right)  
\end{equation}
where $g_\phi$ is the transformation linear layer.
In recommendation settings, item similarity is not as crucial as in image classification task \cite{}. Thus, we adjust sensitivity to item modality variations by tweaking the temperature parameter ($\tau$) in a soft match equation. The loss function to approximate correlation scores is denoted as:
\begin{equation}
    \mathcal{L}^{K D}_{S}=||\sigma\left(r / \tau\right), \sigma\left(r' / \tau\right)||_{l2}
\end{equation}
Here $r$ and $r'$ are predictions from the teacher and student models, respectively, and $l2$ is the square error loss. Raising $\tau$ smooths the probability distribution, reducing disparities. Conversely, decreasing the temperature sharpens the distribution, amplifying the distinctions between probabilities.


\vspace{0.5em}
\noindent \textit{Dissected correlation learning.}
In the teacher model, we employ an unsupervised method—vector quantization—to differentiate various correlation patterns. This approach allows for more nuanced representations but comes with increased computational complexity.
On the other hand, in the student model, we opt for a simpler mechanism to mimic the inter-modal correlation patterns: direct subtraction. This method is computationally more efficient and offers adequate performance for the task at hand. 

For any pair of items, the student model first obtains their directional relationship, specifically the subtraction vector. Based on this subtraction vector, it then predicts the probability distribution $p$ over $K$ classes. This prediction logit $p$ corresponds to the probability of correlation codes provided by the teacher model. Mathematically,
\begin{equation}
    \tilde{e}_{ij} = |e_i - e_j|, \text{~~} p = Out(ReLU(Linear(\tilde{e}_{ij})))
\end{equation}
The teacher's predictions are expressed as a binary distribution, where 1 corresponds to the predicted quantized correlation code, and 0 otherwise. The loss function for the student model can then be formulated as the cross-entropy loss between the student's and teacher's output distributions as shown below.
\begin{equation}
    \mathcal{L}^{K D}_{C}= -\frac{1}{N} \sum_{n=1}^N \sum_{i=1}^K 1(c_{n}=i) \log \left(p_{n, i}\right)
    % \mathcal{L}^{K D}_{C}= -\frac{1}{N} \sum_{n=1}^N \log \left(p_{n, c_n}\right)
\end{equation}
\holden{Should I mention batch size B here?}



% Kernel methods can measure the similarity or relationships between nodes by defining appropriate kernel functions. By selecting the right kernel function $g$, the relationships between nodes can be mapped to d-dimensional vector representations. Common kernel methods include Gaussian kernel, polynomial kernel, and linear kernel (we choose), among others.

% What the student needs to do is simply differentiate the associations between different items, not necessarily to maintain an absolute consistency with the teacher's associations. For example, for 4 nodes, there are 6 pairs of correlations between them. If the teacher’s predicting correlation codes are [1,1,2,1,2,2], the student's task is merely to distinguish between 1 and 2. That is, letting the model realize that the correlations between (suit, tie) and (suit, shoes) is different, thus in the representations centered on "suit", "shoes" and "tie" can be pulled apart. This effectively transforms the multi-class problem into a binary classification problem based on sampling, thereby reducing complexity.

% \subsection{Optimization for Multi-modalities}
% \holden{Add something about Canonical Correlation Analysis (CCA) for Multi-modality}


\subsection{Prediction \& Training Strategy}

% With representation learning modules, as we mentioned in the \textit{Base Model of MSR} in the beginning of this section, we will obtain the hidden states $[h_1, ..., h_n]$ after processing the modality embeddings and ID embeddings. To obtain the final sequence representation $P$ for making a prediction, 
% common methods for this include sum and mean operations on the hidden states $h^l = avg(h_i)_{i=1}^{n}$, which represents the long-term interest representation.


After employing the representation learning modules as outlined in the \textit{Base Model of MSR}, we derive the hidden states $[h_1, ..., h_n]$ or sequence from inputs of modality and ID embeddings. To get the final sequence representation $P$ for prediction, a common approach is to use the mean operation, where $h^l = avg(h_i)_{i=1}^{n}$, indicating the long-term interest representation.

To emphasize short-term interest, we adopt a mix-attention approach for sequence representation. We specifically focus on attention operations solely within the last $q$ items of the sequence. This is represented as:
% However, to highlight the significance of short-term interest, we opt for the mix-attention approach to compute the sequence representation. Specifically, we perform an attention operation exclusively among the last $q$ items in the sequence individually.
\begin{equation}
    \alpha_i = W_2(ReLU(W_1 h_{i})), \text{~}
    h^s = \textstyle\sum_{i=n-q+1}^{n} (\alpha_i h_i) 
    \quad\text{, and}\quad
    P = W_3[h^s; h^l]
\label{eq:short-seq-h}
\end{equation}
$W_1 \in \mathbb{R}^{d \times d}$ and $W_2 \in \mathbb{R}^{d \times 1}$ are two transformation matrix. 
The attention weights, $\alpha \in \mathbb{R}^{q \times 1}$ gauge the significance of the recent items. The short-term interest, $h^s$  is combined with the long-term interest to form the \textbf{final sequence representation}, $P$.
The $W_3 \in \mathbb{R}^{2d \times d}$ is used to project the concatenated short-term interest representation and long-term interest representation.

To supervise the embedding learning with correlation supervision, the overall training target is:
\begin{equation}
    \mathcal{L} = \mathcal{L}^{RS}(y,\hat{y}) + \lambda_1 \mathcal{L}^{KD}_S + \lambda_2 \mathcal{L}^{KD}_C
\end{equation}

\noindent \textbf{Asynchronous training step}
In addition, we consider common adaptation operations where we aim to preserve the original domain's information as much as possible for training new domain parameters to adapt to it.
Taking inspiration from the earlier example with fast decaying modality correlation, we adopt an asynchronous update approach \cite{} for modality embedding parameters and representation parameters. Initially, the updates of modality embeddings are subject to some limitations.
In a word, we aim to control this rapid decay with appropriate correlation constraints and the adaptive training strategy. 



\subsection{Complexity Analysis}
In our study, we propose an optimized process for extracting knowledge from a modality encoder. Our method stands apart from conventional distillation frameworks by pre-processing modality correlations, which facilitates direct and efficient learning for the student model from the teacher. We utilize simple yet effective scoring functions, such as cosine similarity, for gauging correlations, which results in a computational complexity of $O(d)$ for comparisons involving $d$-dimensional vectors. Our method merely adds an extra computation cost of $O(L^2d)$ per sample in both inference and training phases, where $L$ is the length of the training sequence. 
Contrasting our approach with the SASRec with transformer cores and demands $O(L^2dH)$ for representation learning (where $H$ is the attention head), we manage to extract beneficial information from a Large Modality Encoder at a comparably minor multiplicative expense. 

The computational complexity for tuning a Large Modality Encoder, like ResNet, is substantially elevated. Speaking of ResNet, a variant of convolutional neural networks (CNN), its complexity hinges on the network's size and depth. Typically, for a network with L layers, each possessing n feature maps of size h x w, the computational complexity approximates to $O(Lnhw)$ for both the forward and backward passes. Nevertheless, the precise complexity could deviate based on the network's unique architecture and implementation.

==> sec/approach_version2.tex <==
\section{Methodology}

\textbf{Problem Formulation.}
The conventional sequential recommendation aims to predict the next item $v$ a user $u$ is likely to consume, based on their historical interactions $\{v_1, \dots, v_m\}$.
Extending this, Modality-enriched Sequential Recommendation (MSR) considers item modalities within the sequence to refine this predictive function. Specifically, the objective is to acquire a function $f: \{(v_1,a_1,b_1), \dots, (v_m, a_m, b_m) \} \rightarrow v$,
where $a$/$b$ denotes the modality features (image or text) and $a_i$/$b_i$ indicates the modality of item $v_i$ respectively.

In this section, we introduce a novel approach for enhanced modality utilization in MSR through correlation supervision. We outline the framework first, and then give the details of how we implement the correlation distillation \& approximation.


% The goal of conventional \textit{sequential recommendation} can be stated as follows: Given the historical interaction data $\mathbf{H}_u: \{v_1, v_2, \dots, v_m\}$ of user $u$, the objective is to acquire a function $f: \{v_1, v_2, \dots, v_m\} \rightarrow v$ that can predict the next item $v$ that the user is highly likely to consume. 
% Building upon that, modality-enhanced sequential recommendation (MSR) takes into account the modality of items within the sequence, and target to a function that,
% \begin{equation}
%     g: \left\{
%     \begin{aligned}
%     & \mathbf{v}:\{v_1, v_2, \dots, v_m\}, \\
%     & \mathbf{a}:\{a_1, a_2, \dots, a_m\}. 
%     \end{aligned}
%     \right\}
%     \rightarrow
%     \left\{
%     \begin{aligned}
%     & v \\
%     & a 
%     \end{aligned}
%     \right\}
% \end{equation}
% where $a$ denotes the modality features (image or text) we took into consideration.
% Correspondingly, $a_i$ indicates the modality of item $v_i$ respectively.


% \subsection{Base Model of MSR}
% \vspace{0.4em}
% \noindent \textbf{Base Model of MSR.}


\subsection{Overall Framework of Knowledge Distillation for MSR}
\label{sec:pf_basemodel}

% \subsubsection{Base Model.}
Most existing MSR methods adhere to an Encoding, Utilization paradigm, 
% which we term the base model in this section.
as shown in the Figure~\ref{fig:framework}. For simplification and clarity, we use the symbol $a$ in place of $a/b$ when referring to specific modalities in the following.

\vspace{0.5em}
\noindent \textit{Feature Encoding.}
Item ID features $v$ are initially represented as integer index values and can be converted into low-dimensional, dense real-value vectors $\mathbf{e}_v$ using a randomly initialized embedding table. 
Modality feature encoding comprises two key modules: the feature representation module, which represents the original features with vectors $a \rightarrow \mathbf{m}_a$ via modality encoders \cite{he2016deep,raffel2020exploring} pretrained on extensive datasets;
and the embedding initialization module, which adapts these pretrained representations  $\mathbf{m}_a \rightarrow \mathbf{e}_a$ for recommendation tasks.

% Modality $a$'s embeddings often involve directly using extracted features $\mathbf{m}_a$ and representing them as feature vectors $\mathbf{e}_a=\mathbf{m}_a$, through modality encoders \cite{he2016deep,raffel2020exploring}.

\noindent \textit{Feature Utilization.}
Several prior studies have focused on designing network architectures to model feature interactions and generate the overall sequence representation $\mathbf{P}$. Using the \textit{representation learning} function $g$, this is given by:
\begin{equation}
    \mathbf{P} = g(\mathbf{(e_{v_1},e_{a_1}, e_{b_1}), (e_{v_2},e_{a_2}, e_{b_2}),...,(e_{v_m},e_{a_m}, e_{b_m})})
\end{equation}
\noindent \textit{Prediction.}
To match the learned sequence representation $\mathbf{P}$ with candidate items $\mathbf{e}_{v}$, we adopt the wide-used dot product $\hat{y} = \mathbf{P} \cdot \mathbf{e}_{v}^\top$.
% \begin{equation}
% \hat{y} = \mathbf{P} \cdot \mathbf{e}_{v}^\top
% \end{equation}
During training, the model measures the differences between the ground-truth $y$ and the predicted score $\hat{y}$ using the cross-entropy loss \cite{kang2018self}, denoted as $\mathcal{L}^{RS}(y,\hat{y})$.


% \subsubsection{Knowledge Distillation.}
\vspace{0.5em}
\noindent \textbf{Knowledge Distillation.}
As depicted in the Introduction (\S~1), as the training progresses, $\mathbf{e}_a$ will gradually deviate from $\mathbf{m}_a$, leading to the loss of knowledge from the original feature $a$.
This work mainly focuses on how to ensure the initialized embedding $\mathbf{e}_a$ is well utilized.

As shown in the center part bridging the two components in Figure~\ref{fig:framework} (left), we use a common teacher-student paradigm for Correlation Distillation Learning (CDL).
The teacher model distills correlations among items' modalities in the feature encoding stage and then uses it to supervise the student model in the feature utilization stage. 
Formally, the teacher model predicts the correlations between any pair of items $v_i$ and $v_j$, $T(v_i, v_j) = r_{ij}$ concerning their intrinsic modality representations. Similarly, the student model predicts $S(v_i, v_j) = \hat{r}_{ij}$ based on the updated modality embeddings.
In the training phase, the teacher model utilizes its capabilities to guide the student model by minimizing the discrepancy between the outputs $r_{ij}$ and $\hat{r}_{ij}$
In the inference phase, the teacher model is no longer necessary, and the improved student model is employed to make predictions. We will give the details next.

% \textit{Teacher Model -- Modality Correlation Distillation.} 
% Formally, let ${(m_i, m_j, r_{ij})}_{i=1}^N$ be the set of data pairs and corresponding relationships. In this context, the teacher model aims to predict the relationship $r{ij}$ based on the input pairs $(m_i, m_j)$ through the function $f^T(m_i, m_j) = r_{ij}$. In this notation, $m$ represents individual modality features, and $r$ captures their intrinsic correlations.


% \textit{Student Model -- Modality Correlation Learning.} 
% Similarly, the student model aims to predict the distilled correlations based on the updated modality embeddings. Specifically, the function $f^S(e_i, e_j)$ is designed to estimate $r_{ij}$, where $e_i$ and $e_j$ are the updated embeddings for the modalities in question.

% During the training phase, the objective of the student model is to assist in recommendation tasks. This is achieved by minimizing the discrepancy between the outputs generated by the teacher model and those produced by the student model. Formally, the model seeks to minimize the difference between $f^T(m_i, m_j)$ and $f^S(e_i, e_j)$.


\begin{figure}[t]
    \setlength{\abovecaptionskip}{-0cm}
    \setlength{\belowcaptionskip}{-0.5cm}
    \centering
    \includegraphics[width=0.97\textwidth]{fig/framework.png}
    \caption{(left) Framework of KDSR. Green, orange, and blue denote image modality, text modality, and ID features, respectively. (right) Illustration of correlation distillation learning module on image modality.}
    \label{fig:framework}
\end{figure}

% Our paper presents a novel plug-in -- Correlation Distillation (CD) for use with the Base Model, which additionally constrains the correlation among modalities in the base model embedding. As depicted in Figure~\ref{fig:framework}, the Teacher model harnesses abstract knowledge to link modality correlations. Meanwhile, the Student model focuses on learning these distilled correlations for the recommendation system.
% In this section, we first outline the implementation of the unsupervised correlation extraction, i.e., the teacher model. Following that, we explain how these correlations guide the representation of modalities within the embedding space.

\subsection{Bridging the Gap: Correlation Distillation Learning}

As shown in Figure~\ref{fig:framework}~right, two supervision signals are employed: coarse-grained and fine-grained. The teacher distills both signals, and the student approximates them. We will delve into both in the following.

\subsubsection{Modality Correlation Distillation.}
The original $m_i$ derived from the modality encoder is often high-dimensional and laden with redundant data. For discerning refined and distinctive features in representations vectors, we employ a linear AutoEncoder $\mathbf{\tilde{m}}_i = AE(\mathbf{m}_{a_i})$ to convert $\mathbf{m}$ into a streamlined $\mathbf{\tilde{m}}$ first. 
Through such a dimension compression method, it can eliminate redundant features.
Based on these representations, our approach to distilling these correlations spans two distinct perspectives:


\vspace{0.3em}
% \textit{(1) Holistic} correlation scores $T_{s}: \xi(\mathbf{\tilde{m}}_i,\mathbf{\tilde{m}}_j) \rightarrow r_{ij}$.
% We employ an intuitive unsupervised method, using a correlation scoring function $\xi$ to gauge the overarching disparity between paired representations, denoted as continuous value $r$.
% For example, using cosine similarity, the function calculates the angle's cosine between vectors $m_i$ and $m_j$, represented as $\xi(m_i,m_j)=\text{cos}(\theta_{m_i, m_j})$, emphasizing direction over magnitude.
% Given the pivotal role of scoring functions in our study, we offer both distance and similarity-based methods for $\xi$. Their critical importance will be appraised in our experimental section.

\textit{(1) Holistic} correlation scores $T_{s}: \xi(\mathbf{\tilde{m}}_i,\mathbf{\tilde{m}}_j) \rightarrow r_{ij}$.
We use an unsupervised method to determine the disparity between paired representations via the correlation scoring function \( \xi \), yielding a continuous value \( r \). For instance, with cosine similarity, \( \xi(\mathbf{m}_i, \mathbf{m}_j)=\text{cos}(\theta_{m_i, m_j}) \) computes the cosine of the angle between vectors \( \mathbf{m}_i \) and \( \mathbf{m}_j \), prioritizing direction over magnitude. Given the pivotal role of the scoring function in our study, its significance is underscored in our experiment results, showcasing both distance and similarity-based \( \xi \) approaches.

\vspace{0.3em}
\textit{(2) Dissected} correlation codes $T_c: \pi(m_i,m_j) \rightarrow c_{ij}$.
Considering direct vector-wise operations $\xi$ on their vectors are overly simplistic, we provide a fine-grained distillation of discrete correlation signals $c$ through process $\pi$.
Since modality vectors encapsulate varied features like color and shape, a detailed approach is essential to grasp their inherent relationships. 
For instance, while both (\texttt{black-suit}, \texttt{black-tie}) and (\texttt{black-suit}, \texttt{yellow-suit}) pairs might have high correlation scores, the underlying attributes differ. Thus, isolating these distinct correlation patterns into discrete correlation codes is crucial for correlation-type learning.
Specifically, we divide it into two steps -- correlation vectorization and vector quantization.


% Correlation vectorization: 
% Instead of using a single scalar value $r_{i,j}$  to encapsulate the correlation between item modalities  $m_{a_i}$ and $m_{a_j}$, we propose employing a vector $\mathbb{r}_{i,j}$ to capture these relationships in a more fine-grained manner.
% Inspired by the concept of Product Quantization (PQ) \cite{jegou2010product}, we regard each sub-vector as a distinct yet meaningful segment. In this framework, we assume that different positions in the element correspond to unique, meaningful features.
% To begin, we decompose the modality representation vector $m_a$ into $D$ sub-vectors, denoted as $[m_{a,1}, ..., m_{a,D}]$. Following this, we compute the correlation scores (similarity or distance-based) between each sub-vector in $m_{a_i}$ and its counterpart in  $m_{a_j}$. Next, we concatenate these computed metrics to derive correlation vectors. Mathematically, this is expressed as $\mathbb{r}_{i,j} = [\mathbb{r}_{ij,1},...,\mathbb{r}_{ij,D}] = [\xi(m_{a_i,1},m_{a_j,1}), ..., \xi(m_{a_i,D},m_{a_j,D})]$. This methodology enables us to more accurately capture the nuanced relationships between the meaningful segments of the vectors. 

In the first step, rather than representing the correlation between item modalities $m_{a_i}$ and $m_{a_j}$ with a single scalar value $r_{i,j}$, we vectorized their correlations in a vector $\mathbb{r}_{i,j}$.
Drawing inspiration from Product Quantization (PQ) \cite{jegou2010product}, we treat each sub-vector from $m$ as an individual, meaningful segment. In this approach, we posit that unique positions from our streamlined representations correspond to distinct, significant features.
Specifically,
we split the representation vector $m_i$ into $D$ sub-vectors, represented as $[m_{i,1}; ...; m_{i,D}]$. Then we use the scoring function $\xi$ to
measure the correlation scores for each sub-vector in $m_{a_i}$ against its counterpart in $m_{a_j}$. These scores are then concatenated to form correlation vectors, expressed as $\mathbb{r}_{i,j} = [\mathbb{r}_{ij,1},...,\mathbb{r}_{ij,D}] = [\xi(m_{a_i,1},m_{a_j,1}), ..., \xi(m_{a_i,D},m_{a_j,D})]$. Such a method provides a nuanced understanding of the relationships between each vector segment.


In the second step, to further condense the information and encapsulate the correlation pattern more succinctly, we propose to use Vector Quantization (VQ) \cite{hou2023learning} to convert the $N \times N$ correlation vectors $\mathbb{r}_{ij}$, into correlation codes $c_{ij}$. 
This approach can keep conveying the supervision signals, while accommodating minor errors for the imperfect alignment between the encoder's modality spaces and the SR embedding space.
We start by generating a codebook composed of $K$ vectors, where $K$ is a predetermined code number. Each \textit{codeword} in this codebook denotes a potential correlation state. They are initialized randomly, and then optimized with training data to better match the vector distribution of $\mathbb{r}$.
Each vector is then mapped to its nearest codeword, based on Euclidean distance. This process transforms $\mathbb{r} \in \mathbb{R}^{N \times N \times D}$ to $c \in \mathbb{R}^{N \times N \times 1}$, where each entry signifies an index value between 1 and $K$, representing the closest codeword.
In the experiments, we'll also compare other quantization methods.


Using the steps above, similar correlation patterns in the original space are typically mapped to the same codeword, clustering similar correlations. This process also distinguishes subtle patterns, such as "similar color, different shape" versus "similar shape, different color," through distinct codewords, highlighting more nuanced relationships.




% \subsection{Representation Learning}
% Building upon the base model mentioned in Section~\ref{sec:pf_basemodel}, we adopt a decomposed representation approach. This means the ID representing the collaborative information of the item and the modality information representing the features of the item itself are depicted by different vectors.

% Here, it's worth mentioning that in sequence modeling, these decomposed representations intertwine through various fusion methods -- including early fusion, late fusion, and overall fusion. These terms denote whether the fusion of modality features and ID features occurs before or after sequence modeling.

% Let's consider early fusion as an example. For each item, we merge its representations first, denoted as $e_i=merge(e_{v_i},e_{a_i})$, where we use a simple concatenation function for the merge.
% Given the historical interacted item sequence $H_u$ for each user, the representation learning module is responsible for modeling their relationship and producing the updated representation for each item, i.e., $X([e_1,e_2,...,e_n])=[h_1,h_2,...,h_n]$.
% The sequential modeling function $X$ can be any of the following: \textit{Transformer} (SASRec \cite{}), \textit{GRU} (GRU4Rec \cite{}), or a more \textit{intricate graph approach} (RGAT \cite{}).


\subsubsection{Distilled Correlation Approximating.}

To ensure correlation consistency between embeddings $E$ in the modality utilization stage and modality representation $M$ in the modality encoding stage, the student network needs to mirror the outcomes of the complex teacher model. Specifically, we assess item correlation through holistic proximity and directional relations. 
% The details are shown as follows.

\vspace{0.3em}
(1) \textit{Holistic} correlation learning.
In the student model, the correlation between two items $v_i$ and $v_j$ is transformed through their original embeddings, as shown in:
\begin{equation}
    r^{'}_{ij} = \xi \left(g_\phi (a_{i}), g_\phi (a_{j}) \right)  
\end{equation}
where $g_\phi$ is the transformation linear layer.
In recommendation settings, item similarity is not as crucial as in image classification task \cite{}. Thus, we adjust sensitivity to item modality variations by tweaking the temperature parameter ($\tau$) in a soft match equation. The loss function to approximate correlation scores is denoted as:
\begin{equation}
    \mathcal{L}^{K D}_{S}=||\sigma\left(r / \tau\right), \sigma\left(r' / \tau\right)||_{l2}
\end{equation}
Here $r$ and $r'$ are predictions from the teacher and student models, respectively, and $l2$ is the square error loss. Raising $\tau$ smooths the probability distribution, reducing disparities. Conversely, decreasing the temperature sharpens the distribution, amplifying the distinctions between probabilities.


\vspace{0.3em}
(2) \textit{Dissected} correlation learning.
In the teacher model, we employ an unsupervised method—vector quantization—to differentiate various correlation patterns. This approach allows for more nuanced representations but comes with increased computational complexity.
On the other hand, in the student model, we opt for a simpler mechanism to mimic the inter-modal correlation patterns: direct subtraction. This method is computationally more efficient and offers adequate performance for the task at hand. 

For any pair of items, the student model first obtains their directional relationship, specifically the subtraction vector. Based on this subtraction vector, it then predicts the probability distribution $p$ over $K$ classes. This prediction logit $p$ corresponds to the probability of correlation codes provided by the teacher model. Mathematically,
\begin{equation}
    \tilde{e}_{ij} = |e_i - e_j|, \text{~~} p = Out(ReLU(Linear(\tilde{e}_{ij})))
\end{equation}
The teacher's predictions are expressed as a binary distribution, where 1 corresponds to the predicted quantized correlation code, and 0 otherwise. The loss function for the student model can then be formulated as the cross-entropy loss between the student's and teacher's output distributions as shown below.
\begin{equation}
    \mathcal{L}^{K D}_{C}= -\frac{1}{N} \sum_{n=1}^N \sum_{i=1}^K 1(c_{n}=i) \log \left(p_{n, i}\right)
    % \mathcal{L}^{K D}_{C}= -\frac{1}{N} \sum_{n=1}^N \log \left(p_{n, c_n}\right)
\end{equation}
% \holden{Should I mention batch size B here?}




\subsection{Prediction \& Training Strategy}

As shown in Figure~\ref{fig:framework}, the embedding of two modalities and ID will be sent into representation learning modules. 
There are many options, and here we give an example of MMSR \cite{} as the representation learning module, which employs heterogeneous GNN to propagate and exchange information among $e_a$, $e_b$, and $e_v$.
Intermediately, we will get a sequence of hidden states $[h_1, ..., h_n]$ indicates $n$ items.
The final sequence representation \(P\) used in prediction involves long- and short-term aware interests.


% The long-term interest takes the mean, where \(h^l = avg(h_i)_{i=1}^{n}\).
% The short-term interest focuses on attention operations solely within the last $q$ items of the sequence. This is represented as:
% \begin{equation}
%     \alpha_i = W_2(ReLU(W_1 h_{i})), \text{~}
%     h^s = \textstyle\sum_{i=n-q+1}^{n} (\alpha_i h_i) 
%     \text{, and}\quad
%     P = W_3[h^s; h^l]
% \label{eq:short-seq-h}
% \end{equation}
% $W_1 \in \mathbb{R}^{d \times d}$ and $W_2 \in \mathbb{R}^{d \times 1}$ are two transformation matrix. 
% The attention weights, $\alpha \in \mathbb{R}^{q \times 1}$ gauge the significance of the recent items. The short-term interest, $h^s$  is combined with the long-term interest to form the \textbf{final sequence representation}, $P$.
% The $W_3 \in \mathbb{R}^{2d \times d}$ is used to project the concatenated short-term interest representation and long-term interest representation.


For the long-term interest, we compute the mean as \(h^l = avg(h_i)_{i=1}^{n}\).
Conversely, the short-term interest focuses on the last \(q\) items of the sequence, using attention mechanisms. Specifically:
\begin{equation}
    \alpha_i = W_2(ReLU(W_1 h_{i})), \text{~}
    h^s = \textstyle\sum_{i=n-q+1}^{n} (\alpha_i h_i) 
    \text{, and}\quad
    P = W_3[h^s; h^l]
\label{eq:short-seq-h}
\end{equation}
Here, $W_1 \in \mathbb{R}^{d \times d}$ and $W_2 \in \mathbb{R}^{d \times 1}$ are transformation matrices. The attention weights, denoted as $\alpha \in \mathbb{R}^{q \times 1}$, highlight the importance of recent items. By combining the short-term interest \(h^s\) with the long-term interest, we obtain the final sequence representation, \(P\). Lastly, \(W_3 \in \mathbb{R}^{2d \times d}\) projects the concatenated short-term and long-term interest representation.

To supervise the embedding learning using correlation, we incorporate the supervision loss into the prediction loss, resulting in overall training objective:
\begin{equation}
    \mathcal{L} = \mathcal{L}^{RS}(y,\hat{y}) + \lambda_1 \mathcal{L}^{KD}_S + \lambda_2 \mathcal{L}^{KD}_C
\end{equation}

\noindent \textbf{Asynchronous training step}
In addition, we consider common adaptation operations where we aim to preserve the original domain's information as much as possible for training new domain parameters to adapt to it.
Taking inspiration from the earlier example with fast decaying modality correlation, we adopt an asynchronous update approach \cite{} for modality embedding parameters and representation parameters. Initially, the updates of modality embeddings are subject to some limitations.
In a word, we aim to control this rapid decay with appropriate correlation constraints and an adaptive training strategy. 



\subsection{Complexity Analysis}
In our study, we propose an optimized process for extracting knowledge from a modality encoder. Our method stands apart from conventional distillation frameworks by pre-processing modality correlations, which facilitates direct and efficient learning for the student model from the teacher. We utilize simple yet effective scoring functions, such as cosine similarity, for gauging correlations, which results in a computational complexity of $O(d)$ for comparisons involving $d$-dimensional vectors. Our method merely adds an extra computation cost of $O(L^2d)$ per sample in both inference and training phases, where $L$ is the length of the training sequence. 
Contrasting our approach with the SASRec with transformer cores and demands $O(L^2dH)$ for representation learning (where $H$ is the attention head), we manage to extract beneficial information from a Large Modality Encoder at a comparably minor multiplicative expense. 

The computational complexity for tuning a Large Modality Encoder, like ResNet, is substantially elevated. Speaking of ResNet, a variant of convolutional neural networks (CNN), its complexity hinges on the network's size and depth. Typically, for a network with L layers, each possessing n feature maps of size h x w, the computational complexity approximates to $O(Lnhw)$ for both the forward and backward passes. Nevertheless, the precise complexity could deviate based on the network's unique architecture and implementation.

==> sec/intro_version1.tex <==
\section{Introduction}
\label{sec:intro}

% Recommender system (RS) models learn the historical interactions of users and items and recommend items that users may interact with in the future. 

Recommender systems play a crucial role in reducing user overload by helping select preferred items \cite{}.
Sequential Recommenders (SR) specifically focus on learning the sequential relationships among the user's historical items \cite{} and recommend the next items that he/she may interact with. 
SR that utilizes unique identities (IDs for short) to represent distinct items have been well-established and dominated the field for over a decade \cite{}.
Until recently, there has been a paradigm shift towards using modality to represent items, driven by the emergence of sophisticated modality encoders such as Language Language Models (LLM) \cite{?} and advanced high-parameter Image Encoder \cite{?} models.
% These advanced models excel at precisely extracting features and capturing items' inherent correlations from different modalities, such as semantic links in text or visual patterns in images.
These sophisticated models are adept at meticulously extracting features and discerning inherent modalities correlations within items, be it semantic connections in text or visual nuances in images.

% \textbf{[[Break]]}

% Sequential recommendation focuses on modeling the \textit{sequential correlations} (i.e., selection order) between items within sequences. 
SR models encompass from GRU \cite{}, Transformer \cite{}, to Graph Neural Network \cite{}, to model \textit{sequential correlations} (i.e., selection order) between items.
% They aim to better represent items for representation learning based on sequential linkages, thus inherently faces limitations when attempting to leverage the \textit{intrinsic modal correlations} from modality encoders. 
They are designed to optimize item representations for sequential modeling, making them potentially ill-suited for directly leveraging the original modal representations from modality encoders.
% Thus, it inherently faces limitations when attempting to leverage the \textit{intrinsic modal correlations} from modality encoders. 
For the example in Figure~\ref{fig:intro}, considering sequence selection in fashion: people 
usually pick a \texttt{suit} followed by a \texttt{tie}, rather than choosing two visually similar \texttt{suits}. 
Modality encoders can highlight the intrinsic correlations (such as similarity), but they are easily bypassed in SR training, which is more attuned to capturing item sequential relations. This narrow focus undermines SR's ability to understand logical transitions between modalities, leading to poor generalization in unseen cases.


% When leveraging intrinsic modality information, it will pull the representations of various \texttt{suits} closer, and push them away from \texttt{tie}.



Bridging the gap between intrinsic modality correlations 
% (modality correlation for short) 
and item sequential correlation modeling 
% (sequential correlation for short) 
is challenging. 
% Common modality utilization approaches include \textit{end-to-end training} of modality representation learning and recommendation learning. However, this becomes less practical as the parameters of the modality encoder grow, particularly with LLMs and complex convolutional neural networks. 
End-to-end training is a common practice \cite{} utilizing external features, while keeping their original characteristics. But it becomes impractical with growing modality encoder parameters, especially in Large Language Models and other complex Neural Networks.
Increasingly, research is shifting towards efficient two-stage training \cite{}: pertaining encoders first, and then utilizing them with either frozen representations (such as for contrastive learning \cite{zhang2023multimodal} and self-supervised learning \cite{song2023self}), or with unfrozen representations for new recommendation objectives. However, both have limitations.

% The modality embedding-frozen approach lacks flexibility and exhibits a domain gap between the original modality representation and the target item representation \cite{}. In contrast, the modality embedding-unfrozen approach fails to effectively utilize the modal information, leading to \textbf{over-adaptation}. Previous studies \cite{?} have shown that freely training item representations, rather than relying solely on modal initialization or random initialization, does not yield substantial improvements in warm-start tasks. In our pre-experiments shown in Figure~1, we discovered that \textit{during training, the modal representation tends to capture the sequential correlations between items while gradually overlooking their intrinsic visual/semantic correlations.} This could be considered the reason behind our over-adaptation issue. As a result, in the warm-start scenario, relying solely on modalities and ID-based modeling does not yield improvements.


% The frozen modality embedding approach is inflexible \cite{} and persists in a domain gap between original and target item representations. In contrast, the unfrozen approach leads to over-adaptation by failing to capitalize on modal information effectively.
% Without constraints in training, the modality embedding offers little added value over using only IDs in warm-start recommendations \cite{yuan2023go}.
% This over-adaptation issue is evident in our initial experiments in Figure~\ref{fig:intro} (right), where we compare the pair-wise similarities of updated modality embeddings with (standards) to check the information it includes.
%  The standard of original modality correlation is the pair-wise similarities from original modality representations, and we simulate the standard of sequential correlations by measuring the pair-wise similarities of item ID embeddings from another trained pure ID SR model.
%  It can be observed that in training, the modality embedding increasingly incorporates sequential correlations between items. However, the original modality correlation quickly declines to near zero, indicating almost no association.


The frozen modality representation approach lacks flexibility and maintains a adaptation gap between the original and targeted item representations \cite{}. Conversely, the unfrozen methods suffer from over-adaptation due to ineffective use of modal information. 
This issue is demonstrated in our preliminary experiments (Figure~\ref{fig:intro}, right).
We compare the epoch-updated modality embeddings ($E$; initialized by original modality representations) in a modality-enriched SR model with two other standard representation spaces:
($M$) original modality representations including only modal information, and $V$ item embeddings in a separately trained pure ID-based SR model that contains only sequential associations.
% , we employ Pearson Correlation to assess pair-wise similarities between updated modality embeddings ($e$) and two standards: original modality representations ($m$) and item ID embeddings from a separately trained, pure ID-based SR model ($v$).
We employ Pearson Correlation to assess pair-wise item similarities in these spaces.
As training progresses, $E$ increasingly captures sequential item correlations in $V$. However, the correlation with the original modality $M$ rapidly deteriorates to nearly zero, signaling a diminishing relevance to the original modality.
 
% We further validate this over-adaptation issue in our preliminary experiments, as seen in Figure~\ref{fig:intro} (right). 
% The Pearson Correlation evaluates the pair-wise similarities of updated modality embeddings with both (i) original modality representations and (ii) corresponding item ID embeddings in the pure ID model.
% It can be observed that in training, the modality embedding increasingly incorporates sequential correlations between items. However, the original modality correlation quickly declines to near zero, indicating almost no association.

 

 % The Pearson Correlation evaluates similarities between updated modality embeddings during training, original modality representations, and item ID embeddings from the pure ID model. 
 % As training progresses, modality embedding tends to favor sequential item correlations, yet the innate modality connection dwindles to nearly non-existent.


\begin{figure}[t]
    \centering
    \setlength{\abovecaptionskip}{-0cm}
    \setlength{\belowcaptionskip}{-0.5cm}
    \subfigure{\includegraphics[width=0.65\linewidth]{fig/intro_example.png}}
    \subfigure{
		\includegraphics[width=0.33\linewidth]{fig/intro.pdf}}
    \caption{(left) Diagram of adaptation from original modality representation to modality embedding over training epochs. (Right) Experiment on the Beauty dataset with GRU-based models, highlighting the issue of over-adaptation.}
    \label{fig:intro}
\end{figure}


As modality embeddings readily over-adapt to sequential correlations, reducing their distinct advantage over plain IDs \cite{yuan2023go}, we propose to use the teacher-student knowledge distillation paradigm \cite{hinton2015distilling}.
Specifically, the teacher model distills correlations from modality encoders, then uses them to guide the embedding learning during student training.
% However, there are still challenges that exist: 
We further propose designs to solve few challenges:
(1) 
Typically, knowledge distillation (KD) uses a pre-trained teacher model, but an inadequately trained teacher can misguide, causing slow convergence and trapping the model in local optima. To counter this, we adopt an unsupervised method letting the teacher model autonomously discern item correlations. By using an autoencoder, we compress the feature space to capture essential patterns for correlation distillation.
% (2) The modality representations contain valuable information, such as shape, color (for image modalities), high-level category, and brand (for text modalities). Merely relying on overall similarity to express their correlations is inadequate. Therefore, we break the generic correlations into holistic correlation (overall evaluation) and dissected correlation (detailed relationship), blending these two levels of insight.
(2) 
Modality representations contain rich information, encompassing aspects like shape and color in images or high-level category and brand in texts. Solely depending on overall associations (e.g., similarity) for their correlations is insufficient. We thus differentiate correlations into holistic (overall assessment) and dissected (specific types), merging insights from both levels.
(3)
Information from the teacher model isn't always beneficial. To boost accuracy, we deploy a soft-matching strategy aligning teacher's and student's predictions with some allowance for discrepancies. For the dissected correlation, we leverage a vector quantization method, permitting some prediction error in capturing the relationship."


% (x) Regarding the fast dilution of modal information, we apply asynchronous learning rates.

% We conduct experiments across five diverse scenarios with image and text modalities as feature sets. 
We conducted experiments across five distinct scenarios using image and text modalities. 
Our proposed Correlation Distillation Learning (CDL) effectively addresses the swift dilution of modal information, outperforms the top baselines by ~?\% on average.
Additionally, we introduce an asynchronous training step strategy that prevents the early loss of original modal details during training, further offering an enhanced adaptation. 
Our approach is highly compatible with different encoders and SR backbones.
Notably, our method aligns with all large-scale modality encoders, like Swin \cite{} and LLaMA \cite{}. As these encoders grow in size, our quantization technique consistently extracts richer insights. However, a particular embedding dimension is crucial for balancing modal correlation with sequential modeling.

% Additionally, an asynchronous training strategy we introduced prevents premature loss of modality details, enhancing modality adaptation. 

% Regarding the fast dilution of modal information, our proposed Correlation Distillation Learning (CDL) 可以更好地保证模态信息被利用到。并且我们提出了一种asychronous training step的策略--也能更好地在避免在训练前期快速丢失模态原始信息。这是一种更好的模态利用adaptation的策略 -- our approach performs highly compatible and can improve upon the best baselines by ~?\% in average.

% Crucially, our proposed approach suited for all large-scale modality encoders (e.g., Swin, LLaMA). This means efficiently leveraging large encoders for sequential recommendations is not a problem -- As these encoders grow in parameter size, the quantization technique consistently mines richer information.
% 但是值得注意的是，And a certain embedding dimension is required to simultaneously accommodate both modal correlation and sequential modeling.


% Our method is adaptable to multi-modality tasks, where different modality correlations guide their respective modality embeddings. 
% While sequence length impacts sequential models, which vary in their capability to model long and short sequences, our approach performs highly compatible and can improve upon the best baselines by ~?\% in average.
% Crucially, our proposed Correlation Distillation Learning (CDL) suited for all large-scale modality encoders (e.g., Swin, LLaMA). This means efficiently leveraging large encoders for sequential recommendations is now feasible.
% As these encoders grow in parameter size, our correlation quantization consistently mines richer information, ensuring enhanced supervision and consistent performance gains.
% And a certain embedding dimension is required to simultaneously accommodate both modal correlation and sequential modeling.
% Considering the dilution of modal information over time, 


% Our contributions are summarized as follows:
Our contributions are as follows:
% (i) Faced with increasingly large modality encoders, we propose a lighter and more flexible method to preserve the original modality correlation information.
(i) We spotlight challenges of rapid modal information dilution, and propose a knowledge distillation framework to preserve the original modal information.
(ii) We offer a light solution that combines coarse and fine-grained correlation supervision in embedding learning. 
(iii) We conduct comprehensive experiments, which show our solution can keep pace with the rapid evolving modality encoders. It is also practical for a variety of real multi-modal scenarios.
The code of our implementations and baselines will be released for public use \footnote{http://github.com/AnonymousPubCode/ECIR24-CDSRec}.

% In this paper, we propose a novel plugin named as Correlation Distillation (CD) module for augmenting sequential recommendation.
% Different from prior modality-enriched recommendation, which either utilizes frozen modality representation or tune modality representation unguided, we utilize the information from modality encoder through a more flexible way.


==> sec/intro_version2.tex <==
\section{Introduction}
\label{sec:intro}

% Recommender system (RS) models learn the historical interactions of users and items and recommend items that users may interact with in the future. 

Recommender systems reduce user overload by helping them select preferred items \cite{}.
Sequential Recommenders (SR) specifically focus on learning the sequential relationships among the user's historical items \cite{} and recommend the next items that he/she may interact with. 
SR that utilizes unique identities (IDs for short) to represent distinct items have been well-studied and dominated the field for over a decade \cite{}.
Until recently, there has been a paradigm shift towards using modality to represent items, driven by the emergence of sophisticated modality encoders such as Language Language Models (LLM) \cite{?} and advanced high-parameter Image Encoder \cite{?} models.
These sophisticated models are adept at meticulously extracting features and discerning inherent modalities correlations within items, be it semantic connections in text or visual nuances in images.

\holden{Direct transition: Howerver, direct usage of modality feature has a gap in SR.}
SR models, ranging from GRU \cite{}, Transformer \cite{} to Graph Neural Network \cite{}, are designed to model \textit{sequential correlations} (i.e., selection order) between items.
They are specifically designed to optimize item representations for sequential modeling, making them ill-suited for directly leveraging the original modal representations (containing intrinsic \textit{modality correlations}) from modality encoders.
For the example in Figure~\ref{fig:intro}, considering sequence selection in fashion: people 
usually pick a \texttt{suit} followed by a \texttt{tie}, rather than choosing two visually similar \texttt{suits}. 
Modality encoders can highlight their modality correlations (such as similarity), but they are easily overshadowed in SR training, which is more attuned to capturing item sequential relations. 


Thus, tuning or aligning modality knowledge to recommender systems is necessary.
% Bridging the gap between intrinsic modality correlations and item sequential correlation modeling is challenging. 
End-to-end training is a common practice \cite{} utilizing external features, while keeping their original characteristics. But it becomes impractical with growing modality encoder parameters, especially in Large Language Models and other complex Neural Networks.
Efficient two-stage training \cite{} is a solution for it:
pertaining encoders to capture original modality representations, and then utilizing them as embeddings for new recommendation objectives. However, the embedding tuning (in the second stage) suffers from over-adaptation due to the ineffective use of modal information. 


This issue is demonstrated with more clear evidence by our illustration (Figure~\ref{fig:intro}, right).
We compare the epoch-updated modality embeddings ($E$; initialized by original modality representations) in a modality-enriched SR model with two other standard representation spaces:
($M$) original modality representations including only modal information, and ($V$) item embeddings in a separately trained pure ID-based SR model that contains only sequential associations.
We employ Pearson Correlation to assess pair-wise item similarities in these spaces.
As training progresses, $E$ increasingly captures sequential item correlations in $V$. However, the correlation with the original modality $M$ rapidly deteriorates to nearly zero, signaling a diminishing relevance to the original modality.
As modality embeddings readily over-adapt to sequential correlations, it reduces their distinct advantage over plain IDs \cite{yuan2023go}.
\holden{Try to put the descriptions into figure title}

% HC: picture and text say the same: red line ..., and blue line ...


\begin{figure}[t]
    \centering
    \setlength{\abovecaptionskip}{-0cm}
    \setlength{\belowcaptionskip}{-0.5cm}
    \subfigure{\includegraphics[width=0.63\linewidth]{fig/intro_example.png}}
    \subfigure{
		\includegraphics[width=0.35\linewidth]{fig/intro.pdf}}
    \caption{(left) Diagram of adaptation from original modality representation to modality embedding over training epochs. (Right) Experiment on the Beauty dataset with GRU-based models, highlighting the issue of over-adaptation.}
    \label{fig:intro}
\end{figure}

Given concerns above, we introduce a teacher-student knowledge distillation approach \cite{hinton2015distilling} that embraces both merits: it retains the modality feature preservation of end-to-end training while maintaining the high-efficiency characteristic of two-stage training.
Specifically, the teacher model distills correlations from modality encoders, and then uses them to guide the embedding learning during student training.
% However, there are still challenges that exist: 
We further propose designs to solve a few challenges:
(1) 
Typically, knowledge distillation (KD) uses a pre-trained teacher model, but an inadequately trained teacher can misguide, causing slow convergence and trapping the model in local optima. To counter this, we adopt an unsupervised method letting the teacher model autonomously discern item correlations. By using an autoencoder, we compress the feature space to capture essential patterns for correlation distillation.
% (2) The modality representations contain valuable information, such as shape, color (for image modalities), high-level category, and brand (for text modalities). Merely relying on overall similarity to express their correlations is inadequate. Therefore, we break the generic correlations into holistic correlation (overall evaluation) and dissected correlation (detailed relationship), blending these two levels of insight.
(2) 
Modality representations contain rich information, encompassing aspects like shape/color in images or category/brand in texts. Solely depending on overall associations (e.g., similarity) for their correlations is insufficient. We thus differentiate correlations into holistic (overall assessment) and dissected (specific types), merging insights from both levels.
(3)
Information from the teacher model isn't always beneficial. To boost accuracy, we deploy a soft-matching strategy aligning teacher's and student's predictions with some allowance for discrepancies. For the dissected correlation, we leverage a vector quantization method, permitting some prediction error in capturing the relationship."


% (x) Regarding the fast dilution of modal information, we apply asynchronous learning rates.

% We conduct experiments across five diverse scenarios with image and text modalities as feature sets. 
We conducted experiments across five distinct scenarios using image and text modalities. 
Our proposed Correlation Distillation Learning (CDL) effectively addresses the swift dilution of modal information, and outperforms the top baselines by ~?\% on average.
Additionally, we introduce an asynchronous training step strategy that prevents the early loss of original modal details during training, further offering an enhanced adaptation. 
Our approach is highly compatible with different encoders and SR backbones.
Notably, our method aligns with all large-scale modality encoders, like Swin \cite{} and LLaMA \cite{}. As these encoders grow in size, our quantization technique consistently extracts richer insights. However, a particular embedding dimension is crucial for balancing modal correlation with sequential modeling.

% Additionally, an asynchronous training strategy we introduced prevents premature loss of modality details, enhancing modality adaptation. 

% Regarding the fast dilution of modal information, our proposed Correlation Distillation Learning (CDL) 可以更好地保证模态信息被利用到。并且我们提出了一种asychronous training step的策略--也能更好地在避免在训练前期快速丢失模态原始信息。这是一种更好的模态利用adaptation的策略 -- our approach performs highly compatible and can improve upon the best baselines by ~?\% in average.

% Crucially, our proposed approach suited for all large-scale modality encoders (e.g., Swin, LLaMA). This means efficiently leveraging large encoders for sequential recommendations is not a problem -- As these encoders grow in parameter size, the quantization technique consistently mines richer information.
% 但是值得注意的是，And a certain embedding dimension is required to simultaneously accommodate both modal correlation and sequential modeling.


% Our method is adaptable to multi-modality tasks, where different modality correlations guide their respective modality embeddings. 
% While sequence length impacts sequential models, which vary in their capability to model long and short sequences, our approach performs highly compatible and can improve upon the best baselines by ~?\% in average.
% Crucially, our proposed Correlation Distillation Learning (CDL) suited for all large-scale modality encoders (e.g., Swin, LLaMA). This means efficiently leveraging large encoders for sequential recommendations is now feasible.
% As these encoders grow in parameter size, our correlation quantization consistently mines richer information, ensuring enhanced supervision and consistent performance gains.
% And a certain embedding dimension is required to simultaneously accommodate both modal correlation and sequential modeling.
% Considering the dilution of modal information over time, 


% Our contributions are summarized as follows:
Our contributions are as follows:
% (i) Faced with increasingly large modality encoders, we propose a lighter and more flexible method to preserve the original modality correlation information.
(i) We spotlight the challenges of rapid modal information dilution, and propose a knowledge distillation framework to preserve the original modal information.
(ii) We offer a light solution that combines coarse and fine-grained correlation supervision in embedding learning. 
(iii) We conduct comprehensive experiments, which show our solution can keep pace with the evolving modality encoders. It is also practical for a variety of real multi-modal scenarios.
The code of our implementations and baselines will be released for public use \footnote{http://github.com/AnonymousPubCode/ECIR24-CDSRec}.

% In this paper, we propose a novel plugin named as Correlation Distillation (CD) module for augmenting sequential recommendation.
% Different from prior modality-enriched recommendation, which either utilizes frozen modality representation or tune modality representation unguided, we utilize the information from modality encoder through a more flexible way.


==> sec/pre.tex <==
\section{Preliminaries}

\textbf{Problem Formulation.}
The goal of conventional \textit{sequential recommendation} can be stated as follows: Given the historical interaction data $\mathbf{H}_u: \{v_1, v_2, \dots, v_m\}$ of user $u$, the objective is to acquire a function $f: \{v_1, v_2, \dots, v_m\} \rightarrow v$ that can predict the next item $v$ that the user is highly likely to consume. 
Building upon that, modality-enhanced sequential recommendation (MSR) takes into account the modality of items within the sequence. The objective is to obtain a function that,
\begin{equation}
    g: \left\{
    \begin{aligned}
    & \mathbf{v}:\{v_1, v_2, \dots, v_m\}, \\
    & \mathbf{a}:\{a_1, a_2, \dots, a_m\}. 
    \end{aligned}
    \right\}
    \rightarrow
    \left\{
    \begin{aligned}
    & v \\
    & a 
    \end{aligned}
    \right\}
\end{equation}
, where $a$ is a modality feature we took into consideration.
Correspondingly, $a_i$ indicates the image or text of item $v_i$ respectively.
This situation can be seen as equivalent as a process where a large graph in the left-hand side predicts a smaller graph in the right-hand side.
We thus come up with a solution with graph pooling to pool the information from the large graph, generating a more dense graph.



\subsection{Framework of Knowledge Distillation for MSR}
\label{sec:pf_basemodel}
The modality-enriched SR (MSR) can be divided into two main modules: the modality encoding module and the modality utilization module. The encoding module is used to identify useful information from the huge corpus, while the utilization module is responsible for applying external knowledge to recommendation tasks.

\vspace{0.4em}
\noindent \textbf{Base Model of MSR.}
In this section, we first debrief the base model, which follows an Embedding \& Representation Learning \& Prediction paradigm, commonly employed in most existing SRs.

\textit{Initial Embedding.}
Item ID features $v$ are initially represented as integer index values and can be converted into low-dimensional, dense real-value vectors $\mathbf{e}_v$ using a randomly initialized embedding table. Modality $a$'s embeddings often involve directly using extracted features $\mathbf{m}_a$ and representing them as feature vectors $\mathbf{e}_a=\mathbf{m}_a$, through modality encoders \cite{he2016deep,raffel2020exploring}.

\textit{Representation Learning.}
Several prior studies have focused on designing network architectures to model feature interactions and generate the overall sequence representation $\mathbf{P}$. This can be mathematically expressed as:
\begin{equation}
    \mathbf{P} = f(\mathbf{e_v,e_a,...})
\end{equation}

\textit{Prediction.}
The widely-used scoring method involves matching the learned user representation $\mathbf{P}$ with candidate items $\mathbf{e}_{v}$ using the dot product:
\begin{equation}
\hat{y} = \mathbf{P} \cdot \mathbf{e}_{v}^\top
\end{equation}
During training, the model measures the differences between the ground-truth $y$ and the predicted score $\hat{y}$ using the cross-entropy loss \cite{kang2018self}.



\vspace{0.4em}
\noindent \textbf{KD for MSR.}
As the training progresses, $e_a$ will gradually deviate from $m_a$, leading to the loss of modality-specific knowledge.
To fulfill the knowledge gap between the two modules, the process of distillation is used. This process involves using a teacher model to extract valuable knowledge from the encoding module and then using that knowledge to supervise the student model in the utilization module. During the training phase, the teacher model utilizes its capabilities to guide the student model, providing valuable feedback and helping it to learn from its errors. Following the completion of the training phase, the teacher model is no longer necessary, and the improved student model is employed to make predictions.

\textit{Teacher Model.} 
Formally, given $\{(m_i, m_j, r_{ij})\}_i^N$ as the pairs of inputs and target outputs of the teacher model. Here $m$ and $r$ indicate some important linkage within the modality encoder. In our case, $m$ indicates individual modality features and $r$ indicates their intrinsic correlations.
And the teacher model predicts $f^T(m_i, m_j)=r_{ij}$.

\textit{Student Model.} 
In the training phase, the student model aims to aid recommendation objectives by regularizing the difference between outputs from teachers and outputs from students.
Formally, it aims to minimize $(f^T(m_i, m_j), f^S(e_i, e_j))$.

